Retrieving-to-Answer: Zero-Shot Video Question Answering with Frozen Large Language Models

Video Question Answering (VideoQA) has been significantly advanced from the scaling of recent Large Language Models (LLMs). The key idea is to convert the visual information into the language feature space so that the capacity of LLMs can be fully exploited. Existing VideoQA methods typically take two paradigms: (1) learning cross-modal alignment, and (2) using an off-the-shelf captioning model to describe the visual data. However, the first design needs costly training on many extra multi-modal data, whilst the second is further limited by limited domain generalization. To address these limitations, a simple yet effective Retrieving-to-Answer (R2A) framework is proposed.Given an input video, R2A first retrieves a set of semantically similar texts from a generic text corpus using a pre-trained multi-modal model (e.g., CLIP). With both the question and the retrieved texts, a LLM (e.g., DeBERTa) can be directly used to yield a desired answer. Without the need for cross-modal fine-tuning, R2A allows for all the key components (e.g., LLM, retrieval model, and text corpus) to plug-and-play. Extensive experiments on several VideoQA benchmarks show that despite with 1.3B parameters and no fine-tuning, our R2A can outperform the 61 times larger Flamingo-80B model even additionally trained on nearly 2.1B multi-modal data.

==> tables/RetVSCap.tex <==
\begin{table}[t]
    \centering
    \adjustbox{width=\linewidth}{
    \begin{tabular}{@{}ccccc@{}}
        \toprule
        Method & MSRVTT-QA & MSVD-QA & ANet-QA & TGIF-QA \\
        \midrule
        Generated captions & \textbf{18.4} & 32.0 & 25.6 & \textbf{54.6} \\
        Retrieved captions (ours) & 17.6 & \textbf{36.1} & \textbf{26.2} & 50.3 \\
        \bottomrule
    \end{tabular}
    } % adjustbox
    % \vspace{-2mm}
    \caption{{\bf Retrieved captions vs generated captions} }
    % \vspace{-2mm}
    \label{tab:prompt}
\end{table}


==> tables/ft_ctx_length.tex <==
\begin{table}[t]
    \centering
    \adjustbox{width=\linewidth}{
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        max len. & MSRVTT-QA & MSVD-QA & ANet-QA & TGIF-QA \\
        \midrule
        32 \\
        64 \\
        128 \\
        256 \\
        \bottomrule
    \end{tabular}
    } % adjustbox
    \caption{{\bf Effects of max sequence length for vision-language fine-tuning.} The training dataset size is 500k. We scale the batch size accordingly so that the total number of tokens on each GPU is 4096. We only change the number of captions for {\it training} and for evaluation we always use 20 retrieved tokens and a max length of 500 tokens.}
    \label{tab:ft_ctx_length}
\end{table}

==> tables/ft_mlm_prob.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        prob. & MSRVTT-QA & MSVD-QA & ANet-QA & TGIF-QA \\
        \midrule
        0.1 \\
        0.3 \\
        0.5 \\
        \bottomrule
    \end{tabular}
    \caption{{\bf Effects of probability to alter a token during vision-language fine-tunning.}}
    \label{tab:ft_mlm_prob}
\end{table}
